The Farthest Point Map on the Regular Dodecahedron

Let $X$ be the regular dodecahedron, equipped with its intrinsic path metric. Given $p \in X$ let $G(p)=-q$ where $q$ is the point on $X$ which maximizes the distance to $p$. (Generically, $G$ is single-valued.) We give a complete description of the map $G$ and as a consequence show that the $\omega$-limit set of $G$ is the $1$-skeleton of a subdivision of $X$ into $180$ convex quadrilaterals. $G$ is a piecewise bi-quadratic map, and each algebraic piece is defined by a straight line construction involving a rhombus. The rhombi involved have the same shapes as the ones in the Penrose tiling. Our proof is computer-assisted but rigorous.

==> 4stable.tex <==
\section{The Calculations}
\label{struct}


\subsection{Structural Stability}
\label{sv}

We will be considering functions on $T$,
the fundamental domain.  It will be more
convenient to deal with functions on the
unit square $[0,1]^2$.  So, we explain a convenient
map from $[0,1]^2$ to $T$.
 We define
\begin{equation}
  \label{varchange}
  (x,y)=\phi(a,b)=\bigg(a+\frac{1}{4}(1-a)b,\frac{\sqrt 3}{4}(1-a)b\bigg).
\end{equation}
Here $\phi$ is a surjective polynomial map from
$[0,1]^2$ to $T$ which maps $(0,1)^2$
onto $T^o$.  We get $\phi$
by composing the map $(a,b) \to (a,ab)$
with an affine map from the
triangle with vertices $(0,0)$, $(1,0)$, $(1,1)$ to $T$.

We first prove the Structural Stability Lemma for $p \in T^o$.
The combinatorics of the Voronoi decomposition can
change only if one of the edges of the cell decomposition
collapses to a point.  The only edges for which this
can happen are those joining consecutive points on
the list $(012)$, $(025)$, $(235)$, $(345)$.
Such an edge collapses if and only if one of the quadruples
$(0125)$, $(0235)$, $(2345)$ is such
that the corresponding vertices are equidistant
from a single point -- i.e. co-circular. We rule this out.

As is well known, $4$ distinct points $z_1,z_2,z_3,z_4 \in \C$ are
co-circular only if
\begin{equation}
  \chi(z_1,z_2,z_3,z_4)={\rm Im\/}\big((z_1-z_2)(z_3-z_4)\overline{(z_1-z_3)(z_2-z_4)}\big)=0.
\end{equation}
This function is the imaginary part of the cross ratio.
(It also vanishes when the points are collinear.)
Thus, it suffices to prove that
the $3$ functions
\begin{equation}
  \label{precompute}
  T_{ijk\ell}= \frac{16}{27\sqrt 3}  \chi(p_i,p_j,p_k,p_{\ell}) \circ \phi,
\end{equation}
corresponding to the quads above
never vanish on $(0,1)^2$. The
factor out in front is included to make the formulas below nicer.
Now we give formulas for the vertices of $H_p$.  Let
\begin{equation}
  Z(k_1,\ell_1,k_2,\ell_2;p)=w(k_1,\ell_1) p + w(k_2,\ell_2),
  \hskip 20 pt
  w(k,\ell)=\frac{k+\ell \sqrt{3} i}{2}.
\end{equation}
We have $p=p_0=x+iy$, and then a careful inspection of Figure 2.2 gives us
\begin{enumerate}
\item $p_1=Z(-1,+1,+3,-1;p)$.
\item $p_2=Z(-1,-1,+9,+1;p)$.
\item $p_3=Z(+2,+0,+9,+3;p)$.
\item $p_4=Z(-1,+1,+3,+5;p)$.
\item $p_5=Z(-1,-1,+0,+4;p)$.
\end{enumerate}
We plug this in to Equation \ref{precompute} and
factor using
Mathematica [{\bf Wo\/}]:
\begin{equation}
  \label{fact1}
  T_{0125}=(a-1)b\nu_{1}, \hskip 13 pt
  T_{2345}=(1-a)b \nu_{2}, \hskip 13 pt
  T_{0235}=24 a (a-1) (b-1).
\end{equation}
Here, $\nu_1$ and $\nu_2$ are positive on $[0,1]^2$:
$$
\begin{array}{l}
\nu_1=  (8  - 4 a^2 - b^2)+ (8a-4 a b  - a^2 b^2) +  (2 b + 2a^2 b + 2ab^2)\\
\nu_2=  (16 a - 2 a b - 2 a^2 b - 2 a b^2) + (4+a^2 b^2 + 4 a^2 + 4 b + b^2) \\
\end{array}
$$
Hence our $3$ functions in Equation \ref{fact1} are positive on $(0,1)^2$.
This completes the proof when $p \in T^o$.

For the boundary case, we just have to see that there is no
$p \in \partial T$ such that the
cells $C_{i_1},...C_{i_k}$ meet at a point
and less than $3$ of these indices
come from one of the $4$ triples above.
If this happens, then by continuity the
same thing happens when $p$ is perturbed into $T^o$.
Hence, this does not happen.  This proves
the Structural Stability Lemma in the boundary case.
\newline
\newline
    {\bf Remark:\/} The case when $p$ lies in the interior of the
    bottom edge of $T$ corresponds to $b=0$ and $a \in (0,1)$.
    In this case, $T_{0235} \not =0$. This means that $(012)$ and
    $(235)$ are distinct in this case.




\subsection{The Vertex Competition}
\label{final}
\label{final2}

In this section we calculate the function $G$ from \S \ref{sts2}.
Using the formulas for the vertices listed above, we compute the
relevant bisectors and the relevant intersections of these
bisectors to arrive at formulas for the essential vertices.
Here they are.
  
  $$
\begin{array}{cc}
 (012)= \frac{3 \sqrt{3} x^2-6 y x-11 \sqrt{3} x+21 y+5 y^2 \sqrt{3}+8 \sqrt{3}}{2 \left(\sqrt{3} x^2-3 \sqrt{3} x+3 y+y^2 \sqrt{3}+2 \sqrt{3}\right)} 
  +i \frac{3 x^2-2 \sqrt{3} y x-15 x-3 y^2-\sqrt{3} y+12}{2 \left(\sqrt{3} x^2-3 \sqrt{3} x+3 y+y^2 \sqrt{3}+2 \sqrt{3}\right)} \\
  \\
  (025)=\frac{2 \sqrt{3} y^2+2 x y-3 y+3 x \sqrt{3}-8 \sqrt{3}}{2 \left(y+x \sqrt{3}-2 \sqrt{3}\right)} 
  +i \frac{2 y^2-2 \sqrt{3} x y+3 \sqrt{3} y+3 x-12}{2 \left(y+x \sqrt{3}-2 \sqrt{3}\right)} \\
  \\
  (235)=\frac{\sqrt{3} y^2+x y+3 y+3 x \sqrt{3}+2 \sqrt{3}}{y+x \sqrt{3}+\sqrt{3}} +i  \frac{y^2-\sqrt{3} x y+6 x+3}{y+x \sqrt{3}+\sqrt{3}} \\
  \\
  (345)=\frac{3 \sqrt{3} x^2+8 \sqrt{3} x-3 y+y^2 \sqrt{3}+4 \sqrt{3}}{\sqrt{3} x^2+3 \sqrt{3} x-3 y+y^2 \sqrt{3}+2 \sqrt{3}} 
  +i\frac{6 x^2+2 y \sqrt{3} x+15 x+6 y^2-2 \sqrt{3} y+6}{\sqrt{3} x^2+3 \sqrt{3} x-3 y+y^2 \sqrt{3}+2 \sqrt{3}} \\
\end{array}
$$

For $G$ we don't make the change of variables, but rather
compute in terms of $p=x+iy \in T^o$. We have
$$G(x+iy)=-\frac{18 H(x+iy)}{\left(\sqrt{3} x+y-2 \sqrt{3}\right)^2 \left(\sqrt{3} x+y+\sqrt{3}\right)^2},$$
where
$$
H(x+iy)=\left(
\begin{array}{c}
 3 x^5-6 x^4-9 x^3+15 x^2-3 x \\
 3 \sqrt{3} x^4-4 \sqrt{3} x^3-6 \sqrt{3} x^2-3 \sqrt{3} x+\sqrt{3} \\
 2 x^3-6 x^2+15 x-2 \\
 2 \sqrt{3} x^2-2 \sqrt{3} \\
 - x + 4 \\
 -\sqrt{3} \\
\end{array}
\right) \cdot \left(\begin{array}{c} 1 \\ y \\ y^2 \\ y^3 \\ y^4 \\ y^5
\end{array}\right)
$$
The denominator is positive on $T$, so the sign of $H$ determines
the sign of the whole expression.
Using Mathematica to solve the equation $H=0$ for $y$ in terms of $x$, we find that the
solutions are
$$y=\frac{x-1}{\sqrt 3}, \hskip 30 pt
y=\sqrt 3 x,
$$
\begin{equation}
  \label{third}
y=\frac{1}{\sqrt 3} \bigg(1-x- \omega^k((2+x)(5-2x)(1-4x))^{1/3}\bigg).
\end{equation}
Here $\omega=\exp(2 \pi i/3)$ and $k=0,1,2$.
The first two solutions correspond to the
sides of $\partial_{\infty}(T)$.
This third solution intersects $T$ only when
$k=0$.  This is precisely the function in Equation \ref{key},
the one which defines the curve $J$ from
the Main Theorem.  Finally,
$G(1/2)=-1/3$, which shows that
$G$ is positive to the left of $J$ and negative to the right,
when restricted to $T-\partial_{\infty} T$.
This establishes everything we needed to know
about $G$.

\newpage




















==> 5final.tex <==
\section{The Vertex Competition}
\label{final0}


==> Extra/2prelim.tex <==
\section{Preliminaries}

\subsection{A Spatial Argument}

As in the introduction, we let $X$ denote the regular
dodecahedron equipped with its intrinsic path metric.
$X$ is locally Euclidean except for $12$ cone
points, each having cone angle $5 \pi/3$.  As a polyhedron,
$X$ has $12$ {\it faces\/}, each a regular pentagon.
We identify one face $\Pi$ of $X$ with the regular
pentagon whose vertices are the $5$th roots of unity.
We think of $\Pi$ as being the bottom face.
The antipodal face $A(\Pi)$ is the top face.
Geometrically, we are normalizing so that the
distance from the center of a face of $X$ to a
vertex of that face is $1$ unit.

Almost all of our paper uses intrinsic $2$-dimensional
arguments, but there is one spatial argument we give,
in order to shorten the overall proof.  Let us do this
first.  Let  $\phi=(1+\sqrt 5)/2$.  The following facts are well known.
\begin{enumerate}
\item The diameter of any face of
  $X$ is $1+(\phi/2)$.
\item The sphere inscribed in $X$ has radius $\phi^2/2$.
\end{enumerate}

\begin{lemma}
  If $p \in \Pi$ then ${\cal F\/}_p$ is disjoint from the faces
adjacent to $\Pi$.
\end{lemma}

\startproof
Suppose this is false, and
$q \in {\cal F\/}_p$ is in a face adjacent to $\Pi$.
By Fact 1, the points
$p$ and $q$ may be connected to a path of length
at most $2+\phi<4$.  On the other hand,
and path in $X$ connecting $p$ to $A(p)$ stays outside
the inscribed sphere and has endpoints which are
antipodally placed with respect to its center.
Hence, $d_X(p,A(p)) \geq \pi \phi^2/2>4$.
This proves that $A(p)$ is farther from $p$ than is $q$.
Hence $q \not \in {\cal F\/}_p$.
\endproof

\noindent
    {\bf Remark:\/}
    We will eventually show that
    ${\cal F\/}_p \subset A(\Pi)$, but a
    crude argument like the one above would not work
    work to rule out the possibility that ${\cal F\/}_p$
    contains points in the interior of a face adjacent to $A(\Pi)$.
The problem is that the vertex antipodal to any vertex
of $\Pi$ lies both in $A(\Pi)$ and an adjacent face.
\newline

Having finished with the spatial argument, we turn to
more $2$-dimensional considerations.

\subsection{The Developing Map}

Figure 2.1 shows a combinatorial diagram for $X$.
We have $\Pi=\Pi_0$.  The antipodal face
$A(\Pi)=\Pi_{11}$ is not shown.  We have colored the
faces of $X$ according to their combinatorial
distance from $\Pi$.  In the pictures below we will
color $\Pi_{11}$ red.

\begin{center}
\resizebox{!}{2.6in}{\includegraphics{Pix/develop0.eps}}
\newline
    {\bf Figure 2.1:\/} A diagram for the dodecahedron
\end{center}

Figure 2.1 also shows a particular $5$-coloring of the vertices.
This coloring has the property that the vertices of
the same color are the vertices of a regular tetrahedron.
This coloring will help us keep track of the orientations
of the faces when we develop $X$ out into the plane.

A geodesic segment in $X$ cannot have any cone points
in its interior.  For this reason, any geodesic segment
in $X$ is transverse to the edges of $X$ unless it
lies in a single edge of $X$.  We call such a geodesic
segment {\it transverse\/}.  We ignore the geodesic
segments which lie in a single edge of $X$ because
they never arise in connection with the farpoint map.

Let $\gamma^*$ be a transverse geodesic segment
whose initial endpoint lies in $\Pi_0$.
There is a line segment
$\gamma \subset \C$, and an embedded union of
pentagons $$\Pi_{i_0},...,\Pi_{i_k}$$ each sharing a side
with the next, such that $\gamma^*$ and $\gamma$ have
the same length, and $\gamma \cap \Pi=\gamma^* \cap \Pi$.
To cut down on redundancies, we insist that
$i_0=0$ and that otherwise the pentagon chain is
as short as possible.  If the endpoints of
$\gamma$ lie in the interior of faces of $X$ then
the pentagon chain is unique.  The only potential
non-uniqueness arises when the initial
endpoint of $\gamma$ is a vertex of $\Pi_0$, and here
our ``shortest chain'' condition picks out a
chain uniquely in this case.  We will discuss
an example below.

This rolling process is commonly called the
{\it developing map\/}, and $\gamma$ is commonly
called the {\it developing image\/} of $\gamma^*$.
We call $\Pi_0,...,\Pi_{i_k}$ a {\it pentagon chain\/}
and we sometimes refer to it by its associated
sequence $i_0,...,i_k.$
We call the far endpoint of $q$ of $\gamma$ the
{\it terminal point\/}.  Thus, $\gamma$ is the
segment connecting $p$ to $q$, and the
distance from $p$ to $q^*$ {\it along\/}
$\gamma^*$ equals $|p-q|$.

Figure 2.2 shows the $3$ pentagon chains of length
at most $3$ which are associated to minimal
geodesic segments on $X$ connecting a point in
$\Pi_0$ to a point on $\Pi_4$. The associated
sequences are $04$ and $034$ and $054$.

\begin{center}
\resizebox{!}{1.3in}{\includegraphics{Pix/adjacent2.eps}}
\newline
    {\bf Figure 2.2:\/} Chains connecting adjacent faces
\end{center}

The pentagon chains shown in Figure 2.3 do not arise in
connection with a transverse geodesic segment. The only
transverse segment the one on the left could be associated to
starts at the red vertex of $\Pi_0$, but for such geodesic segments the chain does
not have minimal length. The chain $034$ above supports the same segments
and is shorter than $0234$. The chain on the right has a similar story.  The
only potential associated geodesic segments must end at the black
vertex of $X$. The minimal chain in this case would be $036$.

\begin{center}
\resizebox{!}{1.5in}{\includegraphics{Pix/adjacent0.eps}}
\newline
    {\bf Figure 2.3:\/} Two non-minimal chains
    \end{center}

\subsection{Crooked Chains}

More generally, we define a pentagon chain to be any
embedded chain of pentagons with the correct vertex
colorings.  The examples in Figure 2.3 are two
such examples.  We call such a pentagon chain
{\it straight\/} if it contains a line segment
with endpoints in the interiors of the initial
and final faces. We call such a segment
a {\it spanning segment\/}.  We call a chain
{\it crooked\/} if it has no spanning segment.
The chains in Figure 2.3 are
crooked.  A chain arises in connection with
a transverse geodesic segment on $X$ if and only
if it is straight.

One sure-fire way of generating straight chains is to
draw geodesic segments on $X$ and then take the
associated chains.  We do not like this method because
it is hard to check that it is exhaustive.  Our approach
is to list out all possible chain sequences, from the
tree of possibilities (up to a certain length) and
then eliminate the crooked ones.  Here we explain
a computational criterion for crookedness.

Each pentagon chain defines
a finite sequence of segments in the plane,
namely the edges common to consecutive
pentagons in the chain.  We call a list of $3$ edges
{\it bad\/} if there is no line which
intersects all three.  If the pentagon chain
contains a bad triple, then it is crooked.
We can test computationally if a triple
$e_1,e_2,e_2$ is
bad in the following way.  Let $e_{k1}$ and $e_{k2}$
be the endpoints of $e_k$.  If
$e_{21}$ and $e_{22}$ both lie on the same side
of all $4$ lines $\overline{e_{1i}e_{3j}}$
then the triple is bad.

If our test does not show that a chain is
crooked it does not necessarily mean that
the chain is straight.  However, in practice,
we can see immediately that all the
remaining chains have spanning segments.

\subsection{Mirror Images}

We will generally be interested in
pentagon chains whose sequences
start with $0$ and end in either $4$, $9$, or $11$.
(We make these choices somewhat arbitrarily.)
To help us cut down on the enumeration,
we note that the symmetry $I$ of $X$
which preserves the faces
$\Pi_0,\Pi_4,\Pi_9,\Pi_{11}$ has the
following action on chains:
\begin{equation}
  \label{interchange}
  (0,1,2,3,4,5,6,7,8,9,10,11) \leftrightarrow (0,2,1,5,4,3,7,6,10,9,8,11).
\end{equation}
What we mean is that the chains associated
to the geodesics $\gamma$ and $I(\gamma)$ are swapped by the
symbolic map in Equation \ref{interchange}.
This $034$ and $035$ are swapped.  We call such
pairs of swapped chains {\it mirror images\/}.

\subsection{An Example Search}

Here we use a computer search to prove a result
which will be the basis for some other results we prove.

\begin{lemma}
  \label{adjacent}
  The only straight chains of the form $0,...,4$ associated to
  minimal geodesic segments are
    $04$ and $034$ and $054$.
\end{lemma}

\startproof
An exhaustive computer search reveals that there are
$8$ straight pentagon chains of the form $0,...,4$ which
have length $\ell \in \{4,5,6\}$.  These are
$$0,1,8,11,6,4, \hskip 15 pt
0,1,9,10,6,4, \hskip 15 pt
0,1,9,11,6,4 \hskip 15 pt
0,1,9,11,7,4$$
and their mirror images.
Figure 2.4 shows these chains.

\begin{center}
\resizebox{!}{2.8in}{\includegraphics{Pix/adjacent.eps}}
\newline
    {\bf Figure 2.4:\/} Two non-minimal chains
    \end{center}

As we have already mentioned, every
two points in $\Pi_0$ and $\Pi_4$ can be
connected by a path of length at most $2+\phi$.
At the same time, no spanning segment for
any of the chains in Figure 2.4 has length less than
$2+\phi$.  Hence, none of the chains in Figure 2.4
corresponds to a minimal geodesic segment.
The same goes for chains of length $7$ or more,
as one can see by considering the ``tightest'' case,
shown in Figure 2.4, in 
which every three consective pentagons
share a vertex.
\endproof



\subsection{Divide and Conquer}
\label{divide}

There is a second kind of computer search we do.

The triangle $T$ serves as a fundamental
domain for the action of the symmetry
group of $\Pi$.  The left side of
Figure 2.5 shows how $T$ sits in $\Pi$.
The right side shows how we
subdivide $T$ (or indeed any right triangle)
into two smaller right triangles $T_0$ and $T_1$.
We label so that $T_1$ is the triangle
of smaller area.

\begin{center}
\resizebox{!}{.8in}{\includegraphics{Pix/subdivide1.eps}}
\newline
    {\bf Figure 2.5:\/} The triangle $T$ and its subdivision.
    \end{center}

We can iterate this process and arrive
at the triangle $T_{\beta}$ where $\beta$ is
any finite binary sequence.
We say that a {\it triangle product\/} is a
product of the form $T_{\alpha} \times T_{\beta}$,
where both $\alpha$ and $\beta$ are binary
strings.  We associate a parity of such a
product.  The parity is the sum of the lengths
of $\alpha$ and $\beta$.  Thus $T \times T$ is
even and $T_{010} \times T_{0111}$ is odd.

We have a subdivision operation on triangle products.
We define
$$s(T_{\alpha} \times T_{\beta})=(T_{\alpha 0} \times T_{\beta}, T_{\alpha 1} \times T_{\beta}) \hskip 10 pt
{\rm or\/} \hskip 10 pt
s(T_{\alpha} \times T_{\beta})=(T_{\alpha} \times T_{\beta 0}, T_{\alpha} \times T_{\beta 1})$$
according as the triangle product is even or odd.

Suppose we have some computatational property $\Theta$ we want to verify for each
point of $T \times T$.  We will devise a test, involving a finite amount of
computation, which has the following property. If
$T_{\alpha} \times T_{\beta}$ passes the test, then $\Theta$ is true for all
points $(p,q) \in T_{\alpha} \times T_{\beta}$.
We then perform the following algorithm:
\begin{enumerate}
\item Start with a list $L=\{T \times T\}$.
\item If $L$ is empty, {\bf halt\/}. Otherwise, let $\lambda$ be the last member of $L$.
\item If $\lambda$ passes the computational test, omit $\lambda$ from $L$ and return to step 2.
\item If $\lambda$ fails the computational test, omit $\lambda$ from $L$, append
    to $L$ the two members of the subdivision $s(\lambda)$, and return to step 2.
\end{enumerate}
If the algorithm halt it means that all points of $T \times T$ have property $\Theta$.


\newpage









==> Extra/5decagon.tex <==

\section{The Comparison Lemma}

\subsection{A Bound on Displacement}

Our proof of the Comparison Lemma begins with a useful geometric Estimate.
Numericallt, we see that the true bound is closer to $1/22$.  Our method of
proof introduces a bit of slop into the result.

\begin{lemma}[Displacement]
  Assuming that Theorem \ref{main} describes
  $\widehat {\cal G\/}$, we have
  $|p-q|<1/16$ for all $p \in \Pi$ and all
  $q \in \widehat {\cal G\/}_p$.
\end{lemma}

\startproof
Our proof refers to Figure 3.5 and the
Confinement Lemma.
It suffices to prove our
result when $p \in \Sigma_0 \cup \Sigma_1$, the
two states in Figure 3.5.

We first state a geometric principle.
Referring to Figure 1.2,
the difference
\begin{equation}
  \label{increase}
  |z-(R,e,v;z)|
\end{equation}
increases as $z$
moves towards $v$ along the ray $\overrightarrow{vz'}$.
This follows from a similar triangles argument.
Likewise, if we are in the other half of
the domain for the map $(R,e,v)$, meaning
the lower one in Figure 1.2, the quantity
in Equation \ref{increase} decreases as we
move towards $v$ along $\overrightarrow{vz'}$.
We call this the {\it Monotonicity Principle\/}.

Let $(ijk;p)$ denote the triple
point of the Voronoi cell corresponding to the
indices $i,j,k$.  We considered these functions
in \S 3 in detail.

Consider $\Sigma_0$.
By the Monotonicity Principle and symmetry, the restriction of the
$|p-(163;p)|^2$ to the city $C_{163}$ is maximized along the segment $L_0$.
We check in Mathematica that this function is less than $1/256$ on $L_0$.
The same goes for the other three triples $164$, $168$, $169$
respectively associated to $C_{164}, C_{168}, C_{169}$.

The Monotonity Principle combines with the
Confinement Lemma to show that
on the cities $C_{834}$ and $C_{839}$ the respective
functions $|p-(834;p)|^2$ and
$|p-(839;p)|^2$ are bounded above by their
maximum value on the line segment $L_1$.
We check in Mathematica that these functions are
less than $1/256$ on $L_1$.

The Monotonity Principle combines with the
Confinement Lemma to show that
on the cities $C_{831}$ and $C_{836}$ the respective
functions $256|p-(831;p)|^2$ and
$|p-(836;p)|^2$ are bounded above by their
maximum value on the line segment $L_2$.
We check in Mathematica that these functions are
less than $1/256$ on $L_2$.
\endproof

\subsection{Outline of the Proof}

Our goal in this chapter is to prove the Comparison Lemma.
Given the analysis in the previous chapter,
the only pentagon chains corresponding
to minimal geodesic segments joining
$p$ to some point of $A(\Pi)$ are obtained
from appending an $11$ to each of the
basic chain sequences shown in Figure 4.1 or 
taking the image of such a chain, so to
speak, under a symmetry of $X$ which
preserves both $\Pi=\Pi_0$ and $A(\Pi)=\Pi_{11}$.
This gives us $70$ such chains, and we call
these {\it admissible\/}.  We let
${\cal A\/}$ denote the set of these $70$ chains.
Of the $70$ admissible chains, $10$ have
length $4$.  These correspond to the
straightforward geodesic segments.
We call these $10$ chains {\it straightforward\/}.
Let ${\cal S\/}$ denote the collection of $10$
straightforward chains.

    By symmetry it suffices to prove
    the Comparison Lemma for
    $p \in T$, the triangle
    described in \S \ref{divide}.
Assuming that
Theorem \ref{main} describes $\widehat {\cal G\/}_p$, we see
that $p \in T$ implies that $\widehat {\cal G\/}_p \subset T$.
Given $(p,q) \in T^2$ and a chain $C \in {\cal A\/}$, we define
\begin{equation}
\label{deltadef}
  \delta_C(p,q)=|p-q'| \hskip 5 pt {\rm or\/} \hskip 5 pt +\infty.
\end{equation}
Here $q' \in C$ is the unique point in the final pentagon
of the chain that sits in the same position relative to
the vertex coloring as does $A(q)$.  We take the first
option if the line segment $\overline{pq}$ lies in $C$
and we take the second option if not. In the first case,
$\delta_C(p,q')$ is the length of the corresponding geodesic
segment in $X$ connecting $p$ to $A(q)$. In the second case,
there is no geodesic segment corresponding to $C$. So, by definition,
\begin{equation}
  \label{good00}
  \widehat d_X(p,A(q))=\min_{C \in {\cal S\/}} \delta_C(p,q), \hskip 30 pt
  d_X(p,A(q))=\min_{C \in {\cal A\/}} \delta_C(p,q).
\end{equation}

Let ${\cal B\/}$ denote the $60$ chains in ${\cal A\/}$ that do not belong to ${\cal S\/}$.
We call a pair $(p,q)$ {\it good\/} if
\begin{equation}
  \label{good}
  \min_{C \in {\cal S\/}} \delta_C(p,q) \leq
  \min_{C \in {\cal B\/}} \delta_C(p,q).
\end{equation}
To prove the Comparison Lemma it suffices to
prove that $(p,q)$ is good if
$q \in \widehat {\cal G\/}_p$

The picture gets rather complicated near the vertex $1$ of $T$.
Let $$D_1=d_X(1,A(1)=\sqrt{(25/2) + (9/2) \sqrt 5}.$$
There are $24$ members of ${\cal A\/}$ satisfying
$\delta_C(1,1)=D_1$.  Of these chains, $8$ belong to $\cal S$ and
$16$ belong to $\cal B$.  What this means is that
Equation \ref{good} is only barely true near $1$.
We let ${\cal C\/}=\{C_0,...,C_{15}\}$ denote this collection of
$16$ such chains in ${\cal B\/}$, and we treat these chains specially.

Here is our $3$ step proof of the
Comparison Lemma.
\newline
\newline
    {\bf Step 1:\/}
    We use the divide-and-conquer scheme from
    \S \ref{divide} to prove that if $|p-q|<1/16$ then
\begin{equation}
\label{good2} \min_{C \in {\cal S\/}} \delta_C(p,q) \leq
  \min_{C \in {\cal B\/}-{\cal C}} \delta_C(p,q).
\end{equation}
The Displacement Lemma guarantees that this covers
all pairs with $q \in \widehat {\cal G\/}_p$.
\newline
\newline
\noindent
    {\bf Step 2:\/}
    Let $T_{11}$ be the subdivision of $T$ described
    in \S \ref{divide}.  Note that $T_{11}$ is a
    neighborhood of $1$ in $T$. Let $(p,q) \in T^2-T_{11}^2$.
    We prove that if $|p-q|<1/16$ then $(p,q)$
    satisfies Equation \ref{good}.
The Displacement Lemma guarantees that this covers
all pairs with $q \in \widehat {\cal G\/}_p$.
Our estimate here is somewhat delicate.
If we replace $1/16$ with $1/10$ then the
result is false.
 \newline
 \newline
     {\bf Step 3:\/}
     The triangle $T_{11}$ lies entirely in the
cities associated to the triple points $(834)$ and
$(836)$.  We have
\begin{equation}
\widehat d_X(p,\widehat G(p))=|(834;p)-p_8| \hskip 5 pt
{\rm\/} {\rm or\/} \hskip 5 pt |(836;p)-p_8|,
\end{equation}
depending on which city contains $p$.
Let $A_1$ denote the portion of $T_{11}$ above the
line $L_1$ in Figure 5.1. Let $A_2$ denote the
portion of $T_{11}$ below the line $L_2$.
We take $A_1$ and $A_2$ to be closed sets.
For each $k =0,...,15$ we will construct
points $r_k=r_k(p) \in \C$ such that 
\begin{equation}
\delta_{C_k}(p,q)=|q-r_k| \hskip 5 pt
{\rm or\/} \hskip 5 pt +\infty,
\end{equation}
depending on whether $\delta_{C_k}(p,q)$ is
finite or infinite.  We show algebraically that
$$|(834;p)-p_8|<|(834;p)-r_k|$$ on $A_1$ and
$$|(836;p)-p_8|<|(836;p)-r_k|$$ on $A_2$.
These results combine with the Confinement
Lemma and Steps 1 and 2 to finish our proof
of the Comparison Lemma.


\subsection{Setup for the Computational Tests}

We define the {\it control point\/} of a right triangle
to be the midpoint of its hypotenuse. 

Let $\lambda=T_{\alpha} \times T_{\beta}$ be a triangle product.
This is the product of two right triangles.
 We define
$z(\lambda)=(z_{\alpha},z_{\beta})$, where
$z_{\alpha}$ and $z_{\beta}$ are the respective
control points of
$T_{\alpha}$ and $T_{\beta}$.
We define $r_{\alpha}$ and
$r_{\beta}$ to be the respective radii of
$T_{\alpha}$ and $T_{\beta}$.
We call $\lambda$ {\it irrelevant\/} if
\begin{equation}
  |z_{\alpha}-z_{\beta}|-r_{\alpha}-r_{\beta} > \frac{1}{16}.
\end{equation}
If $\lambda$ is irrelevant, then all points $(p,q) \in \lambda$
satisfy $|p-q|>1/16$.

Given a chain $C$ we define
\begin{equation}
\underline \delta_C(\lambda)=\delta_C(z_{\alpha},z_{\beta}) - r_{\alpha}-r_{\beta}.
\end{equation}
Since the map from $z_{\beta}$ to $z_{\beta}'$ is an isometry,
we have 
\begin{equation}
\underline \delta_C(\lambda) \leq \delta_C(p,q), \hskip 15 pt
\forall (p,q) \in \lambda.
\end{equation}

We have to work a bit harder to define our upper bound
$\overline \delta_C$. We say that the pair
$(C,\lambda)$ is {\it compatible\/} if,
for all $9$ vertices $(p,q)$ of $\lambda$, the segment
$\overline{pq'}$ lies in $C$. 
Here $q'$ is as in Equation \ref{deltadef}.

\begin{lemma}
\label{compat}
If $(C,\lambda)$ is compatible, then
$\delta_C(p,q)<\infty$ for all
$(p,q) \in \lambda$.
\end{lemma}

\startproof
Let $e$ be a line segment.  Given
$(u,v) \in \C$ we call
$(e,u,v)$ {\it visible\/} 
if $\overline{uv}$ intersects $e$.
Here is the basic geometric fact.  Suppose
that $\Delta$ is a triangle with vertices
$u,v_1,v_2$.
If $(e,u,v_1)$ and $(e,u,v_2)$ are both visible, then
$(e,u,v)$ is visible for all $v$ in the edge
$\overline{v_1v_2}$.

Call $e$ {\it vertex visible\/} if
$(e,p,q')$ is visible for all $9$ vertices $(p,q)$  of $\lambda$.
Here $q'$ is as in Equation \ref{deltadef}.
Applying the basic fact above several times,
we see that $(e,p,q')$ is visible for all $(p,q) \in \lambda$ provided that $e$ is
vertex visible.

Let $\Pi_0,...,\Pi_{i_k}$ be the pentagons in the chain $C$.
Let $e_1,...,e_k$ denote the edges common
to consecutive pentagons.
Suppose $p \in \Pi_0$ and $q' \in \Pi_{i_k}$. Then
$\overline{pq'} \subset C$
if and only if $(e_j,p,q')$ are visible for $j=1,...,k$.
But this is true iff $e_j$ is vertex visible for all $j=1,...,k$,
and this is true iff $(C,\lambda)$ is compatible.
\endproof

Now we define
\begin{equation}
\overline \delta_C(\lambda)=|z_{\alpha}-z_{\beta}'| + r_{\alpha} +  r_{\beta}
\hskip 5 pt {\rm or\/} \hskip 5 pt +\infty.
\end{equation}
We take the finite value if and only if
$(C,\lambda)$ is compatible.
By Lemma \ref{compat} and the triangle inequality,

\begin{equation}
\label{upper}
\overline \delta_C(\lambda) \geq \delta_C(p,q), \hskip 15 pt
\forall (p,q) \in \lambda.
\end{equation}

Now we define
\begin{equation}
\overline \delta(\lambda)=\min_{C \in {\cal S\/}} \overline \delta_C(\lambda).
\end{equation}
By construction and by Equation \ref{upper}, we have
\begin{equation}
d_X(p,A(q)) \leq \widehat d_X(p,A(q))= \min_{C \in {\cal S\/}} \delta_C(p,q) \leq \overline \delta(\lambda),
\hskip 15 pt \forall (p,q) \in \lambda.
\end{equation}

\subsection{Step 1}

How we describe the computational test for the triangle product
$\lambda$.  First, we return {\bf true\/} if $\lambda$ is irrelevant.
If $\lambda$ is relevant, we do the following.
For each chain $C \in {\cal B\/}-{\cal C\/}$ we
return {\bf false\/} if $\underline \delta_C(\lambda)<\overline \delta(\lambda)$.
If we have not returned {\bf false\/} by the time we have 
tested all chains, we return {\bf true\/}.
A return of {\bf true\/} means that for
all $(p,A(q)) \in \lambda$ we have
$$\min_{C \in {\cal S\/}} \delta_C(p,q) \leq
\overline \delta(\lambda) \leq \min_{C \in {\cal B\/}-{\cal C\/}} \underline \delta_C(\lambda)
\leq \min_{C \in {\cal B\/}-{\cal C\/}} \delta_C(p,q).
$$
In other words, Equation \ref{good2} holds for all $(p,q) \in \lambda$.

When we run the
test it takes about $1$ minute to successfully complete, and
it produces a partition of $T^2$ into $42606$
triangle products which all pass the test.  We will
detail the implementation in \S \ref{formula}.

\subsection{Step 2}

Our test in Step 2 is almost the same as in Step 1,
with two differences.  First, we
define $\lambda=T_{11}^2$ to be
irrelevant. Second, we perform the test with
$\cal C$ in place of the
${\cal B\/}-{\cal C\/}$.
A return of {\bf true\/} means either
that $\lambda = T_{11}^2$ or 
all $(p,q) \in \lambda$ are good.

When we run the
test it takes about $1$ minutes to successfully complete, and
it produces a partition of $T^2$ into $71220$
triangle products which all pass the test.
Again, we will
detail the implementation in \S \ref{formula}.

\subsection{Step 3}
\label{decagon}

\end{document}
\newpage









==> Extra/8formulas.tex <==
\section{Formulas}


\subsection{Transplant Codes}
\label{code}

This section concerns chains whose sequence ends in $11$.
These correspond to geodesic segments which connect a point
in $\Pi$ with a point in $A(\Pi)$.   Given a chain $C$ there
is a $6$ digit {\it transplant code\/}
$(c_0,...,c_5)$ with the following property.
Given $p \in \Pi$ the point $A(p) \in A(\Pi)$ develops
out to the point
\begin{equation}
  \label{transcode}
 \langle C,p \rangle= \sum_{k=0}^4 c_k \exp(2 \pi i k/5) + \exp(\pi i c_5/5) \overline p.
\end{equation}
Here, as usual, we identity $\Pi$ with the pentagon in $\C$
whose vertices are the $5$th roots of unity.
We call $\langle C,p \rangle$ the
{\it transplant\/} of $p$ with respect to $C$.

In our proof of the Correspondence Lemma, we considered
$6 + 60$ chains.  The first $6$ chains let us define
the vertices $p_1,p_3,p_4,p_6,p_8,p_9$ of
the hexagon $H_p$.  The other $60$ chains are the
competing chains which we eliminate.
The point $p_j$ is give by $\langle c_j,p \rangle$, where
\begin{itemize}
  \item $c_1: (0,3,3,1,0,7)$.
  \item $c_3: (3,3,1,0,0,3)$.
  \item $c_4: (3,3,0,0,1,1)$.
  \item $c_6: (3,0,0,1,3,7)$.
  \item $c_8: (0,0,1,3,3,3)$.
  \item $c_9: (0,0,3,3,1,1)$.
\end{itemize}

 Here we $6$ of the sequences corresponding
to the $60$ competing chains and the
corresponding transplant codes.
\begin{itemize}
\item $0,2,1,9,11 \to 2,4,3,0,1,4$
\item $2,10,9,11 \to 1,4,3,2,0,6$
\item $0,3,2,9,11 \to 1,3,4,2,0,6$
\item $0,3,10,9,11 \to 0,2,4,3,1,8$
\item $0,3,2,10,9,11 \to 2,2,5,3,0,7$
\item $0,4,3,10,9,11 \to 0,2,3,5,2,9$.
\end{itemize}
We can deduce the remaining transplant codes
by symmetry.
Given a chain $C$ we define $C^{\#}$ to be the mirror image of $C$.
We define $\omega C$ to be the chain whose developing image
is obtained from that of $C$ by multiplying the whole picture
by $\exp(2 \pi i/5)$.  For instance if the sequence associated
to $C$ is $0,2,9,11$ then the sequence associated to
$\omega C$ is $0,3,10,11$. Given any chain $C$ we have
the $10$  chains $\omega^k C$ and $\omega^k C^{\#}$ for
$k=0,1,2,3,4$. We call these new chains the
{\it dihedral images\/} of $C$.  Here are the rules for figuring out the
transplant codes for the dihedral images.  Assume that $C$ has
transplant code $c_0,...,c_6$ as above. Then...

\begin{enumerate}
\item $C^{\#}$ has transplant code $c_2,c_1,c_0,c_4,c_3,8-c_5$.
\item $\omega C$ has transplant code $c_4,c_0,c_1,c_2,c_3,c_5+4$.
\end{enumerate}





\subsection{Formulas for the City Boundaries}

\label{formula}

  We give formulas for the curves considered above.
  Every formula for a city edge can be obtained from
  the ones below by pre-composing these formulas with
  a dihedral symmetry of the pentagonn $\Pi$.
  We have the relation
  $g_{1683}(x,y)=g_{8316}(x,-y)$, so we won't give the formula explicitly
  for $g_{1683}$. This leaves us with the quadruples above which begin
  with $83$.

  We will simply supply the matrices $\{s_{ij}\}$ and $\{a_{ij}\}$ and $\{b_{ij}\}$ in all
  the relevant cases, and in this order.
  Since it is easy to mix up matrices with their transposes,
    let me say explicitly that the top horizontal row corresponds to the
    monomials $1,x,x^2,x^3$.  With that said, here is the data for
    $g_{8316}$.


{\tiny
\begin{equation}
  \left[\begin{matrix} + & - & - & +\cr + & + & - & 0 \cr -&+&0&0\cr - & 0 & 0 & 0 \end{matrix}\right]
  \hskip 10 pt
  \left[ \begin{matrix} 50 & 585 & 225 & 60 \cr 283 & 12 & 8 & 0 \cr 25 & 40 &0 &0 \cr 8&0&0&0 \end{matrix}\right]
  \hskip 10 pt
 \left[  \begin{matrix} 20 & 171 & -99 & -16 \cr 105 & -4 & 0 & 0 \cr 0 & 40 &0 &0 \cr 8&0&0&0 \end{matrix}\right]
\end{equation}
\/}
Here are the matrices for $g_{8369}$:
{\tiny
\begin{equation}
  \left[\begin{matrix} + & - & - & +\cr + & + & - & 0 \cr -&+&0&0\cr - & 0 & 0 & 0 \end{matrix}\right]
  \hskip 10 pt
  \left[ \begin{matrix} 4700 & 41160 & 210 & 175 \cr 14180 & 1220 & 5 & 0 \cr 2010 & 175 &0 &0 \cr 5&0&0&0 \end{matrix}\right]
  \hskip 10 pt
 \left[  \begin{matrix} 2100 & 18400 & 80 & 75 \cr 6316 & 524 & 1 & 0 \cr 880 & 75 &0 &0 \cr 1&0&0&0 \end{matrix}\right]
\end{equation}
\/}
Here are the matrices for $g_{8349}$:
{\tiny
\begin{equation}
  \left[\begin{matrix} + & - & - & +\cr + & - & + & 0 \cr -&+&0&0\cr + & 0 & 0 & 0 \end{matrix}\right]
  \hskip 10 pt
  \left[ \begin{matrix}   940 & 9480 & 235 & 60 \cr 7780 & 100 &20 &0 \cr 75 &60 &0& \cr 20 &0&0&0 \end{matrix}\right]
  \hskip 10 pt
 \left[  \begin{matrix} 420 & 4400 & 105 & 20 \cr 3476& 44 & -4 & 0 \cr 25 & 20 &0 &0 \cr -4&0&0&0 \end{matrix}\right]
\end{equation}
\/}
Here are the matrices for $g_{8319}$:
{\tiny
\begin{equation}
  \left[\begin{matrix} 0 & - & + & -\cr + & + & - & 0 \cr -& - &0&0\cr - & 0 & 0 & 0 \end{matrix}\right]
  \hskip 10 pt
  \left[ \begin{matrix}   0 & 85 & 130 & 5 \cr 29 & 206 &9 &0 \cr 20 &5 &0& \cr 9 &0&0&0 \end{matrix}\right]
  \hskip 10 pt
 \left[  \begin{matrix} 0 & 38 & 58 &2  \cr 12 & 90 & 4 & 0 \cr 8 & 2 &0 &0 \cr 4&0&0&0 \end{matrix}\right]
\end{equation}
\/}
Here are the matrices for $g_{8346}$:
{\tiny
\begin{equation}
  \left[\begin{matrix} 0 & - & + & +\cr + & + & + & 0 \cr - & + &0&0\cr + & 0 & 0 & 0 \end{matrix}\right]
  \hskip 10 pt
  \left[ \begin{matrix}   0 & 126075 & 58835 & 16810 \cr 109265 & 336200 &16810 &0 \cr 294175 &5 &0& \cr 16810 &0&0&0 \end{matrix}\right]
  \hskip 10 pt
 \left[  \begin{matrix} 0 & 42045 & 25215 &0  \cr 31939 & 26896 & 6724 & 126075 \cr 0 & 2 &0 &0 \cr 6724&0&0&0 \end{matrix}\right]
\end{equation}
\/}

The quadruple point in $\Sigma_0^o$ is
$(\cos(\pi/5)t,\sin(\pi/5)t)$, where  $t=0.25016...$ is a root of the following cubic.
    $$(5 + 3 \sqrt 5) + (-24 - 10 \sqrt 5) t + (-5 + \sqrt 5) t^2 + 4t^3.$$
In the case of the triple points in $\Sigma_1^o$,
I don't know how to prove that the formulas I got from
Mathematica are correct, but I list them anyway.
In the equations below, the list $(a_0,...,a_{10})$ stands for the
polynomial $$a_0+a_1t + ... + a_{10}t^{10}.$$
The two triple points in $\Sigma_1^o$ are the
$$(\cos(2 \pi/5) u_1,\sin(2\pi/5) v_1), \hskip 30 pt
(\cos(2 \pi/5) u_2,\sin(2\pi/5) v_2),$$
where
$u_1,v_1,u_2,v_2$ respectively are the roots of the following
polynomials.
\newline

{\tiny
$$(316255, -1021235 , 1187259 , 628411 , -2861623 , 
  3126530 , -1726141 , 440390 , -15077 , -8998 , 
  604).$$
  
$$(-495, 9045 , -59511, 
  170103 , -171269 , -112328 , 339489 , -267720 , 
  108905 , -25870 , 3020)$$

  $$(-1044164, 
  4232724 , -10713465 , 20137044 , -23128795 , 
  14627289 , -5047850 , 960889 , -66285 , -10636 ,
  724 )$$
  
  $$(-3820, 14590 , 3825 , -149495 , 131854 ,
   97712 , -165546 , -51200 , 15 , -10750 , 
   3620 10)$$
   \/}

To specify the roots exactly it is enough to note that
$$u_1=1.4799...., \hskip 20 pt
v_2=.21542..., \hskip 20 pt u_2=1.4984..., \hskip 20 pt  v_2=.23169...$$

These $4$ degree $10$ polynomials are irreducible, and Sage tells us that
their Galois groups are all degree $2$ extensions of $S_5 \times S_5$ where $S_5$ is the symmetric
group on $5$ symbols. Hence the coordinates for these triple points are
not solvable numbers.    I also found the polynomials for $x_1,y_1,x_2,y_2$.
The formulas for $x_1,x_2$ are similar to the ones for
$u_1,u_2$. The formulas for $y_1,y_2$ are degree $20$ even polynomials with
enormous integer coefficients.


\subsection{Triangle Maps}

In the proof of the
Comparison Lemma and the Voronoi Structure Lemma,
we relied on certain polynomial maps
from $[0,1]^2$ to certain triangles $\Upsilon$
We call these the {\it triangle maps\/}.
Here are the domains
\begin{enumerate}
\item $\Upsilon_0=\Upsilon_{1638}$.  This contains the cities $C_{834}$ and $C_{839}$.
\item $\Upsilon_1=\Upsilon_{8349}$. This contains the cities $C_{831}$ and $C_{836}$.
\item $\Upsilon_{8316}$. This contains the cities $C_{163}$ and $C_{168}$.
\item $\Upsilon_2$. This triangle is such that $\Upsilon_1$ and $\Upsilon_2$ partition the state $\Sigma_1$.
\end{enumerate}


\subsection{The Rhombus Maps}

We will give, in some sense, an algebraic description
of all the maps from Theorem \ref{main} that correspond
to cities in the fundamental domain $T$ described
in \S \ref{divide}.
The formulas for the rhombus maps in Theorem \ref{main} are
rather nasty, but here we explain a method for deriving the
formulas.  One method, of course, is to follow the geometric
definition out to its bitter end.  We describe a more
algebraic method here.

Given two triples
$(R_1,v_1,e_1)$ and $(R_2,v_2,e_2)$, there is a unique
similarity which maps the first triple to the second.
This similarity conjugates the rhombus map based on
the first triple to the rhombus map based on the
second triple.
Accordingly, we first describe the formula for a
prototypical triple $(R_0,v_0,e_0)$ and then we
describe all the triples associated to maps
whose domain is contained in $T$.  We stop
short of actually writing down the similarities.
\newline
\newline
    {\bf Prototypical Example:\/}
    For this example we find it convenient
    to work in $\R^2$ rather than in $\C$.
    We take $R_0=[-1,1] \times [0,2]$,
and $v_0=(-1,0)$ and $e_0$ the vertical
edge connecting $(-1,0)$ to $(-1,2)$.
In this case, the map is given by
\begin{equation}
  f_0(x,y)=\bigg(x,\frac{x^2-1+2y}{y}\bigg).
\end{equation}
Notice that $f_0$ is just barely more
complicated than a projective transformation,
and that $f$ preserves each vertical segment
and acts there as a projective
transformation.
\newline

Now we describe the $6$ triples associated to
maps whose domains lie in $T$.
$s_k=\sin(k \pi/10)$.
Define
$$c_1=s_3-1/2, \hskip 30 pt
x_1=3 s_4, \hskip 30 pt
y_1=3 s_4s_3/s_2.
$$
Let $R_1$ be the rhombus with vertices
$$(c_1, \pm y_1), \hskip 15 pt
(c_1 \pm x_1,0).$$
Up to rotation, this is the ``fat rhombus'' in Figure 1.2.
We have the following.
\begin{itemize}
 \item The triple associated to the mapping $p \to (168;p)$ is
  $(R_1,e,v)$ where $v=(c_1,y_1)$ and $e=\overline{(c_1,y_1)(c_1-x_1,0)}$.
 \item The triple associated to the mapping $p \to (163;p)$ is
  $(R_1,e,v)$ where $v=(c_1,-y_1)$ and $e=\overline{(c_1,-y_1)(c_1+x_1,0)}$.
 \item The triple associated to the mapping $p \to (831;p)$ is
  $(R_1,e,v)$ where $v=(c_1,-y_1)$ and $e=\overline{(c_1,-y_1)(c_1-x_1,0)}$.
 \item The triple associated to the mapping $p \to (836;p)$ is
  $(R_1,e,v)$ where $v=(c_1,y_1)$ and $e=\overline{(c_1,y_1)(c_1+x_1,0)}$.
\end{itemize}

Define
$$c_2=-s_7, \hskip 30 pt
x_2=3 s_7 s_4/s_1, \hskip 30 pt
y_2=3 s_7.
$$
Let $R_2$ be the rhombus with vertices
$$(c_2, \pm y_2), \hskip 15 pt
(c_1 \pm x_1,0).$$
up to rotation, this is the ``thin rhombus'' in Figure 1.2.
Let $\omega=\exp(2 \pi i/5)$.
We have the following
\begin{itemize}
\item The triple associated to the mapping $p \to (834;p)$ is
  $(\omega^3 R_2,\omega^3 v,\omega^3 e)$ where
  $v=(c_2+x_2,0)$ and $e=\overline{(c_2+x_2,0)(c_2,y_2)}$.
\item The triple associated to the mapping $p \to (839;p)$ is
  $(\omega^3 R_2,\omega^3 v,\omega^3 e)$ where
  $v=(c_2-x_2,0)$ and $e=\overline{(c_2-x_2,0)(c_2,-y_2)}$.
  \end{itemize}
This gives a description of all the maps in
the fundamental domain $T$ from
\S \ref{divide}.


\end{document}
 
\newpage



